Learning Regularized Positional Encoding for Molecular Prediction

Machine learning has become a promising approach for molecular modeling. Positional quantities, such as interatomic distances and bond angles, play a crucial role in molecule physics. The existing works rely on careful manual design of their representation. To model the complex nonlinearity in predicting molecular properties in an more end-to-end approach, we propose to encode the positional quantities with a learnable embedding that is continuous and differentiable. A regularization technique is employed to encourage embedding smoothness along the physical dimension. We experiment with a variety of molecular property and force field prediction tasks. Improved performance is observed for three different model architectures after plugging in the proposed positional encoding method. In addition, the learned positional encoding allows easier physics-based interpretation. We observe that tasks of similar physics have the similar learned positional encoding.

==> figures/loss_vs_esz.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/_loss_vs_esz.png}
    % \caption{The dependence of test loss on embedding size, tested on QM9 $U_0$ prediction task with EGNN as the backbone model}
    \includegraphics[width=0.35\textwidth]{figures/_loss_vs_nbin.png}
    \caption{Left: Dependence of test loss on embedding size, tested on QM9 $U_0$ prediction task with EGNN as the backbone model. Right: Dependence of test loss on number of bins, tested on QM9 $U_0$ prediction task with EGNN as the backbone model.}
    \label{fig:emb_size}
\end{figure}

==> figures/loss_vs_nbin.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.43\textwidth]{figures/_loss_vs_nbin.png}
    \caption{The dependence of test loss on number of bins, tested on QM9 $U_0$ prediction task with EGNN as the backbone model}
    \label{fig:n_bin}
\end{figure}

==> figures/overview.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.65\textwidth]{figures/_overview.png}
    \caption{An overview of the proposed learnable regularized position encoding. The learnable embeddings of positional quantities are plugged into neural network molecular predictors. The prediction loss is trained along with a smoothness regularization of embeddings.}
    \label{fig:overview}
\end{figure*}



==> figures/toy.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.6\textwidth]{figures/_toy.png}
    \caption{Comparison of different models on a toy dataset}
    \label{fig:toy}
\end{figure*}

==> figures/turning_point.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.47\textwidth]{figures/_turning_vs_task.png}
    \caption{Distribution of probability of turning points over distance for different tasks}
    \label{fig:turning_point}
\end{figure}

==> sections/2.background.tex <==
\section{Related works}

\subsection{Positional encoding}
There are generally two types of positional encoding, fixed and learned. Fixed positional encoding represent positions with manually picked basis functions. In the initial version of transformer \cite{vaswani2017transformer}, the discrete token positions are represented by a series of sine and cosine functions of a range of fixed frequencies. Gaussian kernels are employed to represent some continuous physical quantities such as interatomic distances in works of molecule modeling \cite{bartok2017machine, chmiela2017machine}. DimeNet \cite{klicpera2020dimenet, klicpera2020dimenetpp} and GemNet~\cite{klicpera2021gemnet} and SphereNet~\cite{liu2021spherical} instead use Spherical Bessel functions and spherical harmonics. Learned positional encoding represent each position with a learned vector. Although initially the fixed positional encoding was proposed for transformers \cite{vaswani2017transformer}, the learnable positional encoding has become more popular technique in natural language processing (NLP) community, as in BERT \cite{devlin2018bert} and GPT models \cite{radford2018gpt1, radford2019gpt2, brown2020gpt3}.
Besides transformers, learnable positional encoding is used with convolutional neural networks \cite{gehring2017convolutional}.

%In contrast to the molecular prediction problems in this work, the previous application of the learned positional encoding are designed for discrete tokens. That technique cannot be directly applied to the continuous positions for molecular modeling.

\subsection{Molecular modeling}

Convolution neural networks are equivariant to translations and this enables them to generalize better on image problems. This characteristic inspires researcher to use them in molecular properties prediction, where translation equivalence is a useful inductive bias. Sch\"{u}tt et.al.
\cite{schutt2017schnet} proposed continuous-filters to apply convolutional layers to molecular modeling tasks from atom-wise features. Miller et.al.
\cite{miller2020l1net} experimented with convolutions that are rotationally invariant as distance and angular features are used. Radial basis function is used to embed pairwise distance. Finzi et.al.
\cite{finzi2020lieconv} proposed a method to construct convolutions equivariant to transformations from a more general groups.

Graph neural networks are another popular family of models used in modeling molecules. 
%This is partially because it is natural to represent the atoms as nodes and their interactions as edges. 
Gilmer et.al.
\cite{gilmer2017nmp} extended the message passing neural networks to predict molecular properties.
The EGNN model \cite{satorras2021egnn} is a graph neural network designed to be equivariant to rotations, translations, reflections and permutations. Each layer takes the distance between pair of atoms and other variables as input. %Instead of using the original distance, we replace it by the proposed distance embedding. 
Other works~\cite{fuchs2020se,dwivedi2021graph} also achieved roto-translational equivariance on GNN or transformers.
The DimeNet++ \cite{klicpera2020dimenetpp} model is an improved version of DimeNet \cite{klicpera2020dimenet}. DimeNet is a graph neural network proposed with focus on the directional message passing in molecule graph. 
%Distance between atoms and angle between pair of atom-atom edges are used as inputs. Spherical Bessel functions and spherical harmonics are used to represent distance and angles. 

There are promising efforts to employ other model architectures in the molecular modeling problems. Anderson et.al.\cite{anderson2019cormorant} proposed a Cormorant network based on neurons designed to be rotationally invariant and takes angular feature into consideration. Ying et.al.
\cite{ying2021graphormer} applied transformers on graph data. They added useful graph features as additional features for token embedding, and modified the attention mechanism considering molecule mechanics.

%The regularized positional encoding method proposed in the present work is a technique that are generally not limited by the choice of neural network architectures reviewd above. As a plug-in module, researchers can replace the raw positional input by the proposed embedding.


==> sections/4.0.toy.tex <==
\subsection{A toy dataset}

\input{figures/toy}

We firstly consider a toy dataset with one dimensional input and output, as illustrated in Figure~\ref{fig:toy}. This is an example where the relation between the input and output is highly nonlinear and non-monotonic. The output can change significantly in a narrow range of the input. 

We encode the input by the proposed positional encoding method (PosEnc), followed by a linear layer. PosEnc divides the input into several bins and this allows great flexibility. As a result, this model fits the toy training data well.
In contrast, both the linear regression model and a Multi-Layer Perceptron (MLP) model underfit this toy dataset. Although in theory MLP is proved to be an universal approximator \cite{cybenko1989approximation}, the performance of the MLP do not become better as we increase the number of layers or hidden units.


==> sections/checklist.tex <==
\section*{Checklist}

\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{see Section~\ref{sec:implement}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{The data is public dataset. The instructions are listed in Section~\ref{sec:implement}. The code will be open-sourced on GitHub}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{see Section~\ref{sec:implement}}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}



==> tables/moleculenet.tex <==
\begin{table}[h]

    \centering
    % https://tex.stackexchange.com/questions/56008/different-sizes-of-font-available-in-table
    \small
    %\footnotesize
    %\scriptsize
    \caption{The performance comparison for molecular properties prediction tasks. The numbers in brackets are the standard deviation.}
    \label{tab:molnet}
    
% \resizebox{0.9\textwidth}{!}
{
\renewcommand{\arraystretch}{1.1}
%\tabcolsep=0.15cm
\tabcolsep=0.06cm
\begin{tabular}{cccccc}
\hline
& \multicolumn{2}{|c}{Classification} & \multicolumn{3}{|c}{Regression }\\
\hline
Dataset & \multicolumn{1}{|c}{Tox21} & {ToxCast} & \multicolumn{1}{|c}{FreeSolv} & {ESOL} & {Lipo} \\
%\# Molecules & \multicolumn{1}{|c}{2039} & {1427} & {1478} & {1513} & \multicolumn{1}{|c}{642} & {1128} & {4200}  \\
%\# Task & 1 & 27 & 2 & 1 \\
\hline
TF\_Robust & 0.698$_{(0.012)}$ & 0.585$_{(0.031)}$  & $4.122 _{(0.085)}$ & $1.722 _{(0.038)}$ & $0.909 _{(0.060)}$ \\
GraphConv  & 0.772$_{(0.041)}$ & 0.650$_{(0.025)}$ & $2.900_{(0.135)}$ & $1.068_{(0.050)}$ & $0.712_{(0.049)}$ \\
Weave  & 0.791$_{(0.008)}$ & 0.678$_{(0.024)}$  & $2.398_{(0.250)}$ & $1.158_{(0.055)}$ & $0.813_{(0.042)}$ \\
SchNet  & 0.767$_{(0.025)}$ & 0.679$_{(0.021)}$  & $3.215_{(0.755)}$ & $1.045_{(0.064)}$ & $0.909_{(0.098)}$ \\
MPNN  & 0.808$_{(0.024)}$ & 0.691$_{(0.013)}$ & $2.185_{(0.952)}$ & $1.167_{(0.430)}$ & $0.672_{(0.051)}$ \\
DMPNN  & 0.826$_{(0.023)}$ & 0.718$_{(0.011)}$  & $2.177_{(0.914)}$ & $0.980_{(0.258)}$ & $0.653_{(0.046)}$ \\
MGCN  & 0.707$_{(0.016)}$ & 0.663$_{(0.009)}$  & $3.349_{(0.097)}$ & $1.266_{(0.147)}$ & $1.113_{(0.041)}$ \\
AttentiveFP  & 0.807$_{(0.020)}$ & 0.579$_{(0.001)}$  & $2.030_{(0.420)}$ &  $0.853_{(0.060)}$ &  $0.650_{(0.030)}$ \\
\hline
EGNN & 
- &     % tox21
- &     % toxcast
1.651$_{(0.137)}$ &     % freesolv
- &     % esol
-  \\   % lipo
\rowcolor{Gray} +PosEnc &
- &     % tox21
- &     % toxcast
1.421$_{(0.239)}$ &     % freesolv
0.651$_{(0.032)}$ &     % esol
0.738$_{(0.072)}$  \\   % lipo
    \rowcolor{Gray} ~~~+Smooth & 
- &     % tox21
- &     % toxcast
- &     % freesolv
- &     % esol
-  \\   % lipo
\hline
\end{tabular}
}
\vspace{-2ex}
\label{tab:properties}
\end{table}

==> tables/table_data.tex <==
\begin{table}[h]
    \centering
    \small
    \begin{tabular}{p{0.2\textwidth}|p{0.12\textwidth}p{0.12\textwidth}} \hline 
                 &  QM9    & PM6 \\ \hline
    train samples & 100 k & 41.0 M \\
    valid samples & 17.7 k & 17.0 k \\
    test samples & 13.0 k & 15.5 k \\ 
    atoms per molecule  & 18.0 & 46.7 \\ 
    number of tasks & 12 & 1 \\
    \hline
    \end{tabular}
    \vspace*{0.1in}
    \caption{Key features of the datasets.}
    \label{table:data}
\end{table}
